AMBER: Automatic Supervision for Multi-Attribute Extraction

The extraction of multi-attribute objects from the deep web is the bridge between the unstructured web and structured data. Existing approaches either induce wrappers from a set of human-annotated pages or leverage repeated structures on the page without supervision. What the former lack in automation, the latter lack in accuracy. Thus accurate, automatic multi-attribute object extraction has remained an open challenge. AMBER overcomes both limitations through mutual supervision between the repeated structure and automatically produced annotations. Previous approaches based on automatic annotations have suffered from low quality due to the inherent noise in the annotations and have attempted to compensate by exploring multiple candidate wrappers. In contrast, AMBER compensates for this noise by integrating repeated structure analysis with annotation-based induction: The repeated structure limits the search space for wrapper induction, and conversely, annotations allow the repeated structure analysis to distinguish noise from relevant data. Both, low recall and low precision in the annotations are mitigated to achieve almost human quality (more than 98 percent) multi-attribute object extraction. To achieve this accuracy, AMBER needs to be trained once for an entire domain. AMBER bootstraps its training from a small, possibly noisy set of attribute instances and a few unannotated sites of the domain.

==> Makefile <==

# $Id: Makefile 4222 2012-10-22 17:44:59Z schallhart $ 

# This makefile builds a number of latex documents sharing the same
# dependencies.
#
# Thus, this makefile is intended either for 
#   * a large document with multiple main-files (e.g. with and without
#     comments), or
#   * a set of simple documents sharing some filees (e.g. macros)
#
# If PDFLATEX is set (to pdflatex), then pdf files are built without
# intermediate postscript files. 
#
#
# The MAIN FILES for all documents are in $tex_files, which defaults
# to the *.tex files in the working directory.
#
# The DEPENDENCIES are taken recursively from 
#   * the paths in $include_path for *.tex, *.dia, *.gnuplot, and *.pdf files
#   * the current working directory for *.bib, *.cls, *.sty, and *.bst
#     files
#   * extra files of these types specified manually
#
# If any of these dependencies changes, all documents from $tex_files
# are to be rebuilt. The latex BUILD first  
#   * converts dia into eps files
#   * runs the gnuplot scripts to obtain pdfs
# and then executes
#   * latex once
#   * bibtex (if a .bbl file has been included)
#   * makeindex (if an index file has been included)
#   * latex once
#   * latex up to 2-4 (depending on latex_rerun) more times, 
#     until cross references are stable 
#
#
#
# The makefile offers GOALS for all documents in $tex_files:
#   * .dvi, .ps, .pdf as usual
#   * .embedded.pdf builds a pdf with all fonts embedded (relies on
#     $papersize)
#
# And it offers the following SUMMARY GOALS:
#   * default/current targets: allps, allpdf, all (usually same as allpdf)
#   * build every target:      totalps, totalpdf, total (usually same as totalpdf)
#   * clean every target:      clean


################################################################################
#
# configuration
#
################################################################################

# The main tex file of the project
# (multiple files allowed---they all share the same dependencies)
tex_files=$(shell ls *.tex)

# the main tex files to be build for target all (restrict this goal, if you
# do not want to build all targets by default)
all_tex_files=$(tex_files)

# include paths for tex and figures
include_path=include figures

# extra bibtex files NOT found recursively in the root directory
bibtex_files=

# extra include files NOT found recursively in the include directories
tex_include_files=
gnuplot_include_files=
dia_include_files=
pdf_include_files=

# extra source files which are NEITHER tex, bib, dia, gnuplot,
# sty, bst, not cls
extra_source_files=

# extra clean files which are NOT caused by tex, dia, or gnuplot files
extra_clean_files=

# papersize for embedded pdf generation
papersize=a4

# the call to latex and pdflatex -- one of them must be there
LATEX=latex
PDFLATEX=pdflatex # -interaction=nonstopmode

# this should determine whether gnuplot exists -- in case tweak manually
# 
# If gnuplot does not exist, the makefile will not produce or delete pdf
# files generated from gnuplot files. Instead, the main build target will
# depend on all _existing_ pdfs generated from the gnuplot files. 
gnuplot_exists=$(shell which gnuplot > /dev/null && echo 1)

# ONE, TWO: one or two runs, with bibtex and makeindex in between
# FOUR: two fixed runs, as above, with two additional optional runs, 
#       which are only performed if there were missing references or
#       citation or the like. 
latex_reruns=TWO

################################################################################
#
# tex, fig, dia, pdf, gnuplot from $include_path
# sty, cls, bst, bib from .
#
################################################################################

# drop the directories which do not exist
include_path_filtered=$(wildcard $(include_path))

extra_source_files+= $(shell find . -name "*.sty")
extra_source_files+= $(shell find . -name "*.cls")
extra_source_files+= $(shell find . -name "*.bst")

bibtex_files+=$(shell find . -name "*.bib")

ifneq ($(include_path_filtered),)
tex_include_files+=$(shell find $(include_path_filtered) -name "*.tex")
ifeq ($(gnuplot_exists),1)
gnuplot_include_files+=$(shell find $(include_path_filtered) -name "*.gnuplot")
endif
dia_include_files+=$(shell find $(include_path_filtered) -name "*.dia")
pdf_include_files+=$(shell find $(include_path_filtered) -name "*.pdf")
endif

################################################################################
#
# derived variables
#
################################################################################

source_files+=$(bibtex_files)

clean_files=$(tex_files:.tex=.bbl) \
            $(tex_files:.tex=.blg) \
            $(tex_files:.tex=.dvi) \
            $(tex_files:.tex=.log) \
            $(tex_files:.tex=.aux) \
            $(tex_files:.tex=.ps)  \
            $(tex_files:.tex=.pdf) \
            $(tex_files:.tex=.sdx) \
            $(tex_files:.tex=.toc) \
            $(tex_files:.tex=.ilg) \
            $(tex_files:.tex=.ind) \
            $(tex_files:.tex=.idx) \
            $(tex_files:.tex=.lot) \
            $(tex_files:.tex=.lof) \
            $(tex_files:.tex=.svn)

clean_files+=$(fig_include_files:.fig=.fig.tex) \
			 $(fig_include_files:.fig=.fig.log) \
			 $(fig_include_files:.fig=.fig.aux) \
			 $(fig_include_files:.fig=.fig.dvi) \
			 $(fig_include_files:.fig=.fig.eps) \
			 $(fig_include_files:.fig=.fig.pstex_t) \
			 $(fig_include_files:.fig=.fig.pstex) 


# dia to eps
dia_pdf_include_files+=$(dia_include_files:.dia=.pdf)
source_files+=$(dia_pdf_include_files)
clean_files+=$(dia_pdf_include_files)

# gnuplot to pdf
gnuplot_pdf_include_files=$(gnuplot_include_files:.gnuplot=.pdf)
pdf_include_files-=$(gnuplot_pdf_include_files)
gnuplot_ps_include_files=$(gnuplot_include_files:.gnuplot=.ps)
source_files+=$(gnuplot_pdf_include_files)
clean_files+=$(gnuplot_pdf_include_files)
clean_files+=$(gnuplot_ps_include_files)

# included tex files
source_files+=$(tex_include_files)
clean_files+=$(tex_include_files:.tex=.aux)

# pdfs 
source_files+=$(pdf_include_files)

# extra include
source_files+=$(extra_source_files)
clean_files+=$(extra_clean_files)

################################################################################
#
# rules (customize)
#
################################################################################

all: allpdf
total: totalpdf

.PHONY: allps allpdf	
allps: $(all_tex_files:.tex=.ps) 
allpdf: $(all_tex_files:.tex=.pdf)

.PHONY: totalps totalpdf	
totalps: $(tex_files:.tex=.ps) 
totalpdf: $(tex_files:.tex=.pdf)


################################################################################
#
# generic rules (do not change)
#
################################################################################

clean:
	rm -f $(clean_files)

# tex -> dvi ###################################################################

latex_needs_rerun_pattern="(There were undefined references|LaTeX Warning: Citation|Rerun to get (cross-references|the bars) right)"
latex_error_report_pattern="(There were undefined references|Rerun to get (cross-references|the bars) right)|undefined|Undefined|Missing|multiply-defined| multiply defined"

%.dvi: %.tex $(source_files)
	@echo
	@echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<"
	@$(LATEX) $(@:.dvi=) </dev/null
	@echo ">>>>>>>>>>> bibtexing $(@:.dvi=) <<<<<<<<<<<"
	@egrep "$(@:.dvi=.bbl)" $(@:.dvi=.log) >/dev/null && bibtex $(@:.dvi=) ; true
	@echo ">>>>>>>>>>> indexing $(@:.dvi=)  <<<<<<<<<<<"
	@egrep "Writing index file" $(@:.dvi=.log) | colrm 1 19 | xargs -n 1 makeindex ; true
ifneq ($(latex_reruns),ONE)
	@echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<"
	@$(LATEX) $(@:.dvi=) </dev/null
ifneq ($(latex_reruns),TWO)
	@egrep $(latex_needs_rerun_pattern) $(@:.dvi=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<" && $(LATEX) $(@:.dvi=) </dev/null; true
	@egrep $(latex_needs_rerun_pattern) $(@:.dvi=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<" && $(LATEX) $(@:.dvi=) </dev/null; true 
endif
endif
	@echo ">>>>>>>>>>> grepped error messages begin: $(@:.dvi=) <<<<<<<<<<<"
	@egrep $(latex_error_report_pattern) $(@:.dvi=.log) | grep -v "Missing character:" ; true
	@echo ">>>>>>>>>>> grepped error messages end: $(@:.dvi=) <<<<<<<<<<<"


# tex -> pdf ##################################################################

ifneq ($(PDFLATEX),)
%.pdf: %.tex $(source_files)
	@echo
	@echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<"
	@$(PDFLATEX) $(@:.pdf=) </dev/null
	@echo ">>>>>>>>>>> bibtexing $(@:.pdf=) <<<<<<<<<<<"
	@egrep "$(@:.pdf=.bbl)" $(@:.pdf=.log) >/dev/null && bibtex $(@:.pdf=) ; true
	@echo ">>>>>>>>>>> indexing $(@:.pdf=)  <<<<<<<<<<<"
	@egrep "Writing index file" $(@:.pdf=.log) | colrm 1 19 | xargs -n 1 makeindex ; true
ifneq ($(latex_reruns),ONE)
	@echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<"
	@$(PDFLATEX) $(@:.pdf=) </dev/null
ifneq ($(latex_reruns),TWO)
	@egrep $(latex_needs_rerun_pattern) $(@:.pdf=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<" && $(PDFLATEX) $(@:.pdf=) </dev/null; true
	@egrep $(latex_needs_rerun_pattern) $(@:.pdf=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<" && $(PDFLATEX) $(@:.pdf=) </dev/null; true
endif
endif
	@echo ">>>>>>>>>>> grepped error messages begin: $(@:.pdf=) <<<<<<<<<<<"
	@egrep $(latex_error_report_pattern)  $(@:.pdf=.log) | grep -v "Missing character:" ; true
	@echo ">>>>>>>>>>> grepped error messages end: $(@:.pdf=) <<<<<<<<<<<"
endif

# simple conversion ############################################################

%.pdf: %.ps
	ps2pdf $< $@

%.embedded.pdf: %.ps
	gs -q -dEmbedAllFonts=true -dNOPAUSE -dBATCH -sPAPERSIZE=$(papersize) \
        -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=$@ -c save pop \
        -f $<

%.ps: %.dvi
	dvips -o $@ $<

%.eps: $.dvi
	dvips -E $< -o $@

# dia -> pdf ###################################################################

$(dia_pdf_include_files): %.pdf: %.dia
	dia -t pdf -e $@ $< 

# gnuplot -> ps, pdf ##########################################################

$(gnuplot_pdf_include_files): %.pdf: %.ps
	epstopdf $<
#	ps2pdf $< $@

$(gnuplot_ps_include_files): %.ps: %.gnuplot
	cd $(dir $@); gnuplot < $(notdir $<) > $(notdir $@)




